Stochastic Gradient Langevin Dynamics with Variance Reduction

Stochastic gradient Langevin dynamics (SGLD) has gained the attention of optimization researchers due to its global optimization properties. This paper proves an improved convergence property to local minimizers of nonconvex objective functions using SGLD accelerated by variance reductions. Moreover, we prove an ergodicity property of the SGLD scheme, which gives insights on its potential to find global minimizers of nonconvex objectives.

==> header.tex <==
\usepackage{amssymb}		% to get all AMS symbols
\usepackage{graphicx}		% to insert figures
\usepackage[hidelinks]{hyperref}		% PDF hyperreferences??

\usepackage{float}
\usepackage{bbm}
\usepackage{bm}
\usepackage{ulem}
\usepackage{extarrows}
\usepackage{enumitem}
\usepackage{comment}
\usepackage{amsthm,amsmath,amsfonts}
\usepackage{mathrsfs}
\usepackage{subcaption}
\usepackage{booktabs}
% \usepackage[colorlinks=true]{hyperref}
% \usepackage[noend]{algorithmic}
% \usepackage[algo2e,ruled,linesnumbered]{algorithm2e}
% This is a bit nicer:
\usepackage{algorithm,algpseudocode} % algorithmicx package
\usepackage{breakcites}
% \usepackage{cleveref}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{assumption}{Assumption}
\newtheorem{remark}[theorem]{Remark}

% \affil{Department of Applied Mathematics}
\usepackage{natbib}
\usepackage{xspace}

% \usepackage[latin1]{inputenc}


%% sketching chapter
\newcommand{\R}{\mathbb{R}}
\renewcommand{\P}{\mathbb{P}}
\newcommand{\dis}{\displaystyle}
\newcommand{\E}{\mathbb{E}\,}
\newcommand{\X}{\mathbf{X}}
\newcommand{\Y}{\mathbf{Y}}
\newcommand{\Z}{\mathbf{Z}}
\newcommand{\x}{\mathbf{x}}
\newcommand{\y}{\mathbf{y}}
\newcommand{\z}{\mathbf{z}}
\renewcommand{\d}{\mathrm{d}}
\newcommand{\A}{\mathcal{A}}
\newcommand{\B}{\mathcal{B}}
\newcommand{\Xtensor}{\mathcal{X}}
\newcommand{\Ytensor}{\mathcal{Y}}
\newcommand{\HD}{\mathbf{HD}}
\newcommand{\e}{\mathrm{e}}
\newcommand{\<}{\langle}
\renewcommand{\>}{\rangle}
\newcommand{\sketch}{\boldsymbol{\Omega}}

\newcommand{\be}{\mathbf{e}}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\bv}{\mathbf{v}} % "b" for bold
\newcommand{\bw}{\mathbf{w}}
\newcommand{\bH}{\mathbf{H}}
\newcommand{\bD}{\mathbf{D}}
\newcommand{\bP}{\mathbf{P}}
\newcommand{\eps}{\varepsilon}
\newcommand{\noise}{\boldsymbol{\epsilon}}
\newcommand{\longT}{T_\text{long}}
\newcommand{\Var}{\mathbb{V}\text{ar}}

% \newcommand{\argmin}[1]{\underset{#1}{\mathrm{argmin} \, }}
\usepackage{tikz}
\newcommand*\circled[1]{\tikz[baseline=(char.base)]{
   \node[shape=circle,draw,inner sep=1pt] (char) {\footnotesize #1};}}
   
\newcommand{\autocorr}{R} % single tau
% \newcommand{\Autocorr}{\mathbf{R}} % all tau
\newcommand{\Autocorr}{\mathbf{R}} % all tau
\newcommand{\transpose}{\intercal} % or ...
% \newcommand{\transpose}{\top}
\newcommand{\trans}{\transpose}
\newcommand{\covmat}{\boldsymbol{\Sigma}}


%% PPD
% \usepackage[usenames,dvipsnames,svgnames]{xcolor}

\newcommand{\diff}{\mathrm{d}}
\newcommand{\n}{\boldsymbol{n}}
\newcommand{\prox}{\mathrm{prox}}
\newcommand{\Lip}{L}  % Lipschitz constant
\newenvironment{longversion}{}{}
\newcommand{\ball}{\mathbb{B}}
\newcommand{\EFSP}{$\varepsilon$-first-order stationary point}
\newcommand{\ESSP}{$\varepsilon$-second-order stationary point\xspace}
\newcommand{\defeq}{\mathrel{\mathop:}=}
\newcommand{\argmin}{\mathop{\rm argmin}}
\newcommand*{\minimize}{\mathrm{minimize}}
\newcommand{\grad}{\nabla}
\newcommand{\hess}{\nabla^2}
\newcommand{\ugrad}{\mathscr{G}}
\newcommand{\ufun}{\mathscr{F}}
\newcommand{\uspace}{\mathscr{S}}
\newcommand{\utime}{\mathscr{T}}
\newcommand{\Ts}{T'}
\newcommand{\Tt}{T''}
\newcommand{\ca}{\hat{c}}
\newcommand{\cn}{\kappa}
\renewcommand{\u}{\mathbf{u}}
\renewcommand{\v}{\mathbf{v}}
\newcommand{\w}{\mathbf{w}}
\newcommand{\logterms}{\frac{d\cn}{\delta}}
\newcommand{\norm}[1]{\|{#1}\|}
\newcommand{\cXs}{\mathcal{X}_{\text{stuck}}}
\newcommand{\proj}{\mathcal{P}}
\renewcommand{\H}{\mathcal{H}}


%% LD-SVRG
\newcommand{\gradsvrg}{\widetilde{\nabla}}
\newcommand{\xbatch}{\widetilde{\x}}
\newcommand{\gradnorm}{\|\nabla _t\|^2}
\newcommand{\fsp}{\x_{\mathrm{fsp}}}
\newcommand{\pr}{\mathbf{Pr}}


%% miscellany
\newcommand{\argmax}{\textrm{arg}\max}
% \newcommand{\argmin}{\textrm{arg}\min}

==> introduction.tex <==
\section{Introduction}
% \textcolor{red}{novelty}

In this chapter we consider the optimization algorithm \textit{stochastic gradient descent} (SGD) with variance reduction (VR) and Gaussian noise injected at every iteration step. For historical reasons, the particular randomization format of injecting Gaussian noises bears the name \textit{Langevin dynamics} (LD). Thus, the scheme we consider is referred as \textit{stochastic gradient Langevin dynamics with variance reduction} (SGLD-VR). We point out the ergodicity property of SGLD-VR schemes when used as an optimization algorithm, which the normal SGD method without the additional noise does not have. As the ergodicity property implies the non-trivial probability for the LD process to visit the whole space, the set of global minima may also be traversed during the iteration, thereby revealing the potential of such a scheme for the purposes of global optimization.  We provide convergence results of SGLD-VR to local minima in similar style as those in \cite{Huang_PPD}.

We apply the SGLD-VR scheme on the empirical risk minimization problem:
\begin{equation}
    \label{prob::LD_main_prob}
    \textrm{minimize } f(\boldsymbol{\omega}) = \frac{1}{n} \sum_{i=1}^n f_i(\boldsymbol{\omega})
\end{equation}
which is a sampled version of the stochastic optimization problem: $\dis \min_{\boldsymbol{\omega}} F(\boldsymbol{\omega}) = \int f(\boldsymbol{\omega};\x)\,\mathrm{d} \x$, where $\x$ is the collection of training data and $\boldsymbol{\omega}$ is the parameter for the model. In the following text we use $\x$ instead of $\boldsymbol{\omega}$ as the input for the objective $f$. For empirical risk minimization, one may construct the gradient estimator by subsampling terms in the summation of the objective \eqref{prob::LD_main_prob} for gradient evaluation in order to accelerate the optimization process, which coincides with the SGD framework. Variance reduction is leveraged to accelerate convergence, and LD is further engaged in the SGD scheme to enable ergodicity property and convergence property to local minima.

\subsection{Prior art}

The Langevin dynamical equation describes the trajectory $X(t)$ of the following stochastic differential equation
\begin{equation}
\mathrm{d}X_t = -\nabla U(X_t)\,\mathrm{d} t + \sigma\,\mathrm{d}B_t,
\end{equation}
which is a characterization for the continuous motion of a particle in a potential field $U$. Using this dynamic as a master equation, through Kramers–Moyal expansion one can derive the Fokker-Planck equation, which gives the spatial distribution of particles at a given time, thus a full characterization of the statistical properties of a particle ensemble \cite{KRAMERS_FK_equation}. 

\paragraph{LD and sampling} The connection between Langevin dynamics (LD) and the distribution of particle ensemble reveals the potential of applying LD on sampling. Suppose that the  distribution of interest is $\pi(\x)$ and that there exists a function $U$ such that $\pi(\x)=\frac{\exp(-U(\x))}{\int\exp(-U(\x))\,\mathrm{d}\x} $, then LD equation which contains a Brownian motion term gives a Monte-Carlo-natured simulation based on the distribution $\pi(\x)$, and the stationary distribution such a dynamic converges to is $\pi(\x)$. To numerically implement LD equation for sampling purposes, one needs to discretize the continuous LD equation. A simple version of the dicretization is the \textit{unadjusted Langevin algorithm} (ULA), 
\begin{equation}
    \x_{k+1} = \x_k - \eta_k\nabla U(\x_k) + \rho_0\sqrt{\eta_k} \noise_k
\end{equation}
where $\noise_k \in \mathcal{N}(0,\mathbf{I}_d)$, $\x\in \R^d$. The Gaussian noise term enables the scheme to explore the sample space and the drift term guides the direction of exploration. One common modified scheme is \textit{Metropolis adjusted Langevin algorithm} (MALA), where upon the suggested update by ULA, there is an additional accept/reject step, with the probability of accepting the the update as $1\wedge\frac{\pi(\x_k)p(\x_k|\x_{k+1})}{\pi(\x_{k+1}) p(\x_{k+1}|\x_k) }$. % MALA assures the convergence to the target distribution, while ULA can lack such a guarantee.

Naturally two central questions related to this sample scheme arise: whether or not the distribution of samples generated by LD converges, and if so, to $\pi$; and what is the mixing time of LD (i.e., how long does it takes for the LD to approximately reach equilibrium hence generating valid samples from the distribution $\pi$).
The first question motivates the importance of MALA: in terms of \textit{total variation} (TV) norm, while ULA can fail to converge for either light-tailed or heavy-tailed target distribution, MALA is guaranteed to converge to any continuous target distribution \cite{MeynTweedie_MC_Book}. Regarding the second question about convergence speed, researchers have investigated the sufficient conditions for ULA and MALA respectively to guarantee exponential (geometric) convergence to target distribution. \cite{MengersenTweedie_MHA} shows for distributions over $\R$, the necessary and sufficient condition for MALA to converge to target distribution $\pi(\x)$ at geometric speed is that $\pi(\x)$ has exponential tails. The sufficiency of this condition is generated to higher dimension in \cite{RobertsTweedie_MHA}.
The seminal work \cite{RobertsTweedie_LD} shows that w.r.t.\ target distributions that are in essence non-localized, or heavy-tailed, MALA cannot converge at geometric speed.

% There have been parallel work investigating sampling with constraints. Following works by \cite{Bubeck_log_concave_sampling} and \cite{Brosse_log_concave_sampling_proximal_LMC} address the constrained sampling problem with LD algorithms, where the former considers the localized convex sample space with an additional projection step within ULA to enforce boundedness, and the latter resorts to using the Moreau envelope of the indicator function to encode the compactness of the sample space. Both of these work, assuming log-concavity of $U$, lead to disadvantageous dependence of time complexity on optimization parameters (the former $\mathcal{O}(\frac{d^{12}}{\eps^{12}})$ and the latter $\mathcal{O}(\frac{d^5}{\eps^6})$). 
% Another effort to address the constrained sampling and to generalize  LD to sample non-log-concave distributions is through the mirrored LD \cite{mirrored_langevin_dyn}, whose central step is to construct the dual distribution which is both log-concave and unconstrained from compactness requirement and then to map back to primal space. The mirrored LD has improved parameter dependence $\mathcal{O}(\frac{d^2}{\eps^2})$.
In parallel there have been works to show the convergence of LD for distribution approximation in terms of Wasserstein-2 distance \cite{dalalyan_LMC_guarantees} and KL-divergence respectively \cite{LMC_convergence_KL}.

A particular case of interest for the application of LD on sampling is to find the posterior distribution of parameters $\boldsymbol{\theta}$ in the Bayesian setting, where the updates are set as
\begin{equation}
\label{eqn::bayesian_theta_update}
\Delta \boldsymbol{\theta}_k = \eta_k \left( \nabla p(\boldsymbol{\theta}_k)  + \sum_{i=1}^N \nabla \log p(\x_i|\boldsymbol{\theta}_k) \right) + \sqrt{\eta_k}\noise_k
\end{equation}
where $\noise_k\sim\mathcal{N}(0,\mathbf{I})$. To maximize the likelihood, \cite{Bayes_learning_SGLD} suggests to use the format of stochastic gradient descent in the derivative term of \eqref{eqn::bayesian_theta_update}. \cite{Borkar_Mitter_1999} shows that this minibatch-styled LD will converge to the correct distribution in terms of KL divergence.

\paragraph{LD and optimization} The main focus of this paper is on optimization. LD offers an exciting opportunity for  global optimization due to the exploring nature of the Brownian motion term. Simulating multiple particles to obtain information about the geometric landscape of the objective function---thus locating a global minimum---is often too computationally expensive to be practical. Notice that when one considers the convergence to a distribution, the exploring nature of LD due to continually injected Gaussian noise of constant variance is the key factor, while for the purpose of optimization, one usually exploits noises with diminishing variance since the goal is to converge to a point. 

The technique to achieve this point convergence is \textit{annealing}, which means decreasing the variance of the noise as $t$ grows. Formally, let the objective function be $U$ and we construct the probability distribution $p_T(\x) = \frac{1}{Z}\exp\left(-\frac{U(\x)}{T} \right)$, where $Z$ is the normalization factor. The key observation is that as the parameter $T\to 0$, the distribution $p_T(\x)$ will concentrate on the global minima. This parameter $T$ is usually referred to as \textit{temperature}, alluding to the alloy annealing process where as temperature decreases, the structure of the metal evolves into the most stable one, hence reaching the state with minimum potential energy. To formulate  LD for optimization, one essentially takes the usual LD equation but with the variance term $\sigma$ now a function of time, $\sigma = \sqrt{T}(t)$:
\[
\mathrm{d}\x_t = \nabla U(\x_t)\,\mathrm{d} t + \sqrt{T(t)}\, \mathrm{d} B_t
\]
The pioneering work by Chiang et al.\   \cite{diffusion_global_optimization_1987} shows that with the annealing schedule $T(t) \propto (\log t)^{-1}$, then  LD will find the global minimum. The work by Chiang et al.\ does not specify how to simulate the continuous version of Langevin dynamics, thus not providing information on the convergence of discrete approximation (Euler-Maruyama method as an example) for LD. \cite{Gelfand_Mitter_1999} fills this gap by proving that with an annealing schedule $\eta_k \propto k^{-1}$ and $T_k\propto (k\log\log k)^{-1}$, then discretized LD will converge to the global minima in probability. More recently, \cite{SGLD_Raginsky} uses optimal transport formalism to study the empirical risk minimization problem. Their proof uses the Wasserstein-2 distance to evaluate distribution discrepancy and consists of two parts: first show that the discretization error of LD from continuous LD accumulates linearly with respect to the error tolerance level, and then show that the continuous LD will converge to the true target distribution exponentially fast.

\paragraph{Variance reduction (VR) and LD} In this paper we aim to apply variance reduction techniques in the setting of LD to acceleration the optimization process and to derive improved time complexity dependence on error tolerance level.

The specific VR technique we use was originally proposed to reduce the variance of the minibatch gradient estimator in stochastic gradient descent for convex objectives by \cite{SVRG} and separately by \cite{SAGA}. \cite{Reddi_SVRG_first_order_2016,allen2016variance} have respectively generalized the application of VR techniques to nonconvex objectives and provided convergence guarantee to first-order stationary points.

In essence, we use the \textit{control variate} technique to construct a new gradient estimator by adding an additional term to the minibatch gradient estimator in SGD ($\nabla_{\mathrm{SGD}}$) and this term is correlated with $\nabla_{\mathrm{SGD}}$, thus reducing the variance of the gradient estimator as a whole. More specifically, consider the classic gradient estimator of function $f$ in \eqref{prob::LD_main_prob} at point $\x$: $\nabla_{\mathrm{SGD}} = \frac{1}{|\mathcal{I}|}\sum_{i\in\mathcal{I}} \nabla f_i(\x)$, where $\mathcal{I}\subseteq[n]$. If there is another r.v.\ $Y$ whose expectation is known, then we can construct a new unbiased gradient estimator $\widetilde{\nabla}$ of function $f$ at point $\x$ as $\widetilde{\nabla} = \nabla_{\mathrm{SGD}} + \alpha(Y-\E Y)$, where $\alpha$ is a constant. If $\alpha = -\frac{\mathrm{Cov}(\nabla_{\mathrm{SGD}},Y)}{\mathrm{Var}[Y]}$, then the variance of new gradient estimator $\widetilde{\nabla}$ is $\mathrm{Var}[\widetilde{\nabla}] = (1-\rho^2_{\nabla_{\mathrm{SGD}},Y})\mathrm{Var}[\nabla_{\mathrm{SGD}}] \le \mathrm{Var}[\nabla_{\mathrm{SGD}}]$, where $\rho$ is the Pearson correlation coefficient between $\nabla_{\mathrm{SGD}}$ and $Y$. Usually one may not be lucky enough to have access to such a r.v.\ $Y$ whose covariance with $\nabla_{\mathrm{SGD}}$ is known, therefore the constant $\alpha$ for the control variate needs to be chosen in an empirical manner.

Motivated by applications in physics and neural network, there has been more interest in guarantees for convergence to second-order stationary points by optimization algorithms.
% , even if in approximate sense. 
A continual line of work has relied on randomized first-order methods, in particular gradient descent \cite{jin2017escape} and proximal descent \cite{Huang_PPD} to achieve this purpose. See the latter for a detailed review for this line of work.
% See section \ref{subsection::opt_method_review} in chapter \ref{chapter::PPD} for a detailed review for this line of work.

The main algorithm we consider in this paper is stochastic gradient Langevin dynamics (SGLD) with variance reduction, which consists of two sources of randomness: one from stochastic gradients, the other from Gaussian noise injected at each step. Previous work have investigated the SGLD for optimization to find local minimizers \cite{Hitting_time_analysis_SGLD_ChenDuTong,Hitting_time_analysis_SGLG_ZhangLiangCharikar}, and reported results for convergence to approximate second order stationary points. In particular, \cite{SGLD_Gu} show that with constant-variance Gaussian noise injected at each step, SGLD-VR finds an approximate minimizer with time complexity $\mathcal{O}(\frac{d^5}{\eps^4})$. We aim to improve the dependency on $\eps$. We also point out that when variance of Gaussian noise is set as constant in SGLD, the function value or the point distance between optimal point and iterate can never go to zero, but can be bounded by a constant depending on the size of variance.

Finally we want to mention that \cite{SVRG_SGLD_crude} introduces the VR technique to Bayesian inference setting where the objective is the posterior and the gradient estimator is constructed with minibatch of training data. However, the given convergence guarantee is in terms of mean squared error of statistics evaluated based on posterior, instead of posterior distribution of the parameter. 

\paragraph{Contribution}
This paper discusses the convergence properties of SGLD with variance reduction and shows the ergodicity property of the scheme. Our main contributions upon the prior art is the following:
\begin{itemize}
    \item We provide a better time complexity for the SGLD-VR scheme to converge to a local minimizer than the corresponding result in \cite{SGLD_Gu}. 
    \item We show the ergodicity property of SGLD-VR scheme based on the framework set for SGLD scheme in \cite{Hitting_time_analysis_SGLD_ChenDuTong}.
\end{itemize}

\begin{table}[H]
\centering
\begin{tabular}{ lcccc } 
\toprule
method & w.\ VR & noise magnitude setting & convergence target & Time complexity $m$\\
\midrule
\cite{SGLD_Raginsky} & no & constant & global min.\ & $\dis  \widetilde{\mathcal{O}}\left( \frac{d+1/\delta_0}{\delta_0\eps^4} \right) $  \\
\cite{SGLD_Gu} & yes & constant & global min.\ & $\dis \widetilde{\mathcal{O}}\left( \frac{1}{\eps^{5/2}} \right)\exp(\widetilde{\mathcal{O}}(d))$\\
\cite{Hitting_time_analysis_SGLG_ZhangLiangCharikar}& no &  constant &  local min.\ & $\dis \mathcal{O}\left( \frac{\Delta_f d^4L^2}{\eps^4} \right)$  \\
This work & yes & diminishing w.\ poly.\ speed & local min.$^*$ & $\dis \mathcal{O}\left(\frac{\Delta_f}{\eps^2}\right) + \exp\left(\mathcal{O}(\eps d)\right) $ \\
\bottomrule
\end{tabular}
\caption{Comparison between convergence results for variants of LD optimization schemes. $^*$ indicates convergence target is actually a $\eps$-second-order stationary point, which coincides with a local minimizer when $\eps < \sqrt{q}$ under assumption \ref{as::strict_saddle_ld}.}
% \addtabletext{nomenclature for the TSs refers to the numbered species in the table.}
\label{table::ld_convergence_comparison}
\end{table}
\paragraph{Notation} Bold symbols indicate vectors, for example a vector $\x\in \R^d$, where $d$ stands for the dimension of Euclidean space.  We use $o$ to indicate the starting index of a minibatch. We use $\eta_{a:b}$ as the shorthand for $\sum_{i=a}^b \eta_{i}$.


% VR technique is used in the setting of maximizing posterior likelihood for Bayesian inference with LD. 
% Variance reduction SVRG (Reddi; Allen-Zhu; Dubey; Bach; )

==> main_result.tex <==


\section{Algorithm and main results}
The main algorithm is given as algorithm \ref{alg::LD}. 
% \textcolor{red}{ finite sum minimization problem for $f$: define $f$}

\begin{algorithm}[ht]
\caption{Variance reduced stochastic gradient Langevin dynamics (VRSGLD)
}%evaluation with sketching}
\label{alg::LD}
\begin{algorithmic}[1]
%           \While{$r\not=0$} \Comment{We have the answer if r is 0}
%           \State
\Require initial stepsize $\eta_0>0$, stepsize decay order $\nu \ge 1$, initial Gaussian noise magnitude parameter $\delta_0$, batch size $B_b$, epoch length $B_{\e}$
% , temperature parameter $\beta_t>0$
\State Initialize $\x_0=0$, $\xbatch^{(0)} = \x_0$
\For{$s=0,1,2,\cdots,\frac{T}{B_{\e}}-1$}
\State $\widetilde{\mathbf{w}} = \nabla f(\xbatch^{(s)})$
\For{$l=0,1,\cdots,B_{\e}-1$}
    \State set index $t=s B_{\e}+l$
    \State randomly pick a subset $I_t$ from $[n]$ of size $|I_t|=B_b$; randomly draw $\noise_t\sim \mathcal{N}(0,\mathbf{I})$
    \State construct gradient estimator $\gradsvrg_t = \frac{1}{B_b} \sum_{i_t\in I_t} \big( \nabla f_{i_t}(\x_t) - \nabla f_{i_t}(\xbatch^{(s)}) + \widetilde{\mathbf{w}} \big)$
    \State update $\x_{t+1} = \x_t - \eta_t \gradsvrg_t + \rho_t \noise_t$
\EndFor
\State $\xbatch^{(s)} = \x_{(s+1)B_{\e}}$
\EndFor

\end{algorithmic}
\end{algorithm}
In algorithm \ref{alg::LD}, the stepsize $\eta_t$ and $\rho_t$ is set as the following, for some  $\nu\ge 1$:
\begin{equation}
\label{eqn::stepsize_LD}
\eta_t = \frac{\eta_0}{t^\nu} \textrm{ and } \rho_t = \frac{\rho_0}{t^{\nu/2}}.
\end{equation}

\paragraph{Ergodicity} In this work we show that the discretized variance reduced LD (VRSGLD) has an ergodic property which gives the iteration process the potential of exploring wider space, thus with positive possibility of traversing through the global optimal point.

The argument for ergodicity has two parts: In Lemma~\ref{lemma::recurrence} we first give an explicit upper bound of the expected time of visiting a given level set for the $j$-th time ($j\ge 1$); then in Theorem~\ref{thm::ergodicity} we show that there is a positive possibility such that the LD iteration can visit any fixed point within a level set.

\begin{assumption}[Lipschitz Gradient]
\label{as::grad_lipschitz_ld}
$f$ is continuously differentiable, and there exists a positive constant $L$ such that for all $\x$ and $\y$, $\|\nabla f(\x) - \nabla f(\y)\|\le L\|\x-\y\|$.
\end{assumption}

\begin{assumption}[Regularization conditions for the objective function $f$]
\label{assumption::regularization_conditions}
There exist non-negative constants $\mu_1$, $\mu_2$ and $\psi_1$, $\psi_2$ such that for all $\x\in\R^d$, 
\begin{align}
\label{ineqn::ergo_regularisation_1}
    \|\nabla f(\x)\|^2 &\ge \mu_1 f(\x) - \psi_1\\
\label{ineqn::ergo_regularisation_2}
    \|\x\|^2 &\le \mu_2 f(\x) + \psi_2
\end{align}
\end{assumption}
\paragraph{Remark} We make the same regularization assumptions as in \cite{Hitting_time_analysis_SGLD_ChenDuTong}. A relevant regularization condition commonly used in previous literature is the \textit{$(m,b)$-dissipative condition} \cite{Mattingly_ergodicity_2002,SGLD_Raginsky,SGLD_Gu,Hitting_time_analysis_SGLG_ZhangLiangCharikar}, which reads that there exist positive constants $m$ and $b$ such that for all $\x\in\R^d$, $\<\nabla f(\x),\x\>\ge m\|\x\|^2-b$. \cite{dong2020replica} shows that the dissipative condition implies \eqref{ineqn::ergo_regularisation_1}, which renders the assumption \eqref{ineqn::ergo_regularisation_1} weaker. Equation \eqref{ineqn::ergo_regularisation_2} implies that $f$ is supercoercive~\cite{CombettesBook2}, and in particular coercive, and thus has bounded level sets.

% Meanwhile, \eqref{ineqn::ergo_regularisation_2} is not independent from \eqref{ineqn::ergo_regularisation_1}.

\begin{lemma}[Recurrence]
\label{lemma::recurrence}
Let $n_0$ be the index such that $\eta_{n_0}\le \delta$, and $n_k$ be the sequence of iteration index $n_{k+1} = \min_s\{ s : s>n_k, \,  \eta_{n_k:s} \ge \delta   \}$. 

Under the regularization conditions in Assumption \ref{assumption::regularization_conditions} and under Assumption \ref{as::grad_lipschitz_ld}, there exists a constant $C_1$ such that $\alpha = 1-2\exp(-(1-C_1)\mu\delta)$, $B = 2(\frac{2\eta_0 L^3}{B_\e}f(\x_0) + \frac{\delta_0^2 Ld}{2\eta_0})$ and $K = \frac{\ln\frac{f(\x_{n_0})}{\delta B}}{(1-C_1)\mu\delta}$, with the stopping time sequence $\{\tau_k\}$ defined as $\tau_{0}=K$ and $\tau_{k+1} = \min\{t: t\ge \tau_k + 1, f(\x_{n_t})\le 2\delta B\}$, 
\begin{equation}
    \E[\tau_j] \le \frac{4}{\alpha} + K + j\left(\frac{1}{2\alpha\delta }+1\right)
\end{equation}
\end{lemma}

% Then we show that there is a positive possibility such that the LD iteration can visit any fixed point within a level set.

\begin{theorem}[Ergodicity]
\label{thm::ergodicity}

Under the regularization conditions in Assumption \ref{assumption::regularization_conditions} and under Assumption \ref{as::grad_lipschitz_ld}, with the same parameter setting as in Lemma \ref{lemma::recurrence}, for any accuracy  $\widetilde{\eps}>0$, failure probability $p>0$,  and any point $\mathbf{s}\in\R^d$, there is a number 
\begin{equation}
    T = \mathcal{O}\left(\frac{1}{p\mu_1\big(4\eta_0L^3 \frac{\mu_2 f(\x_0) + 2\psi_2}{B_\e} + \frac{\delta_0^2}{\eta_0} Ld\big)}\left(1 + \ln f(\x_0)   + \frac{(d\|\mathbf{s}\| + \widetilde{\eps}) ^d }{ \big( (\frac{4}{\sqrt{2\pi}}-1)\mathrm{e}^{-1/2} \widetilde{\eps} \big)^d}  \right) \right)
\end{equation} such that
\begin{equation}
    \pr(\|\x_t - \mathbf{s}\|\le \widetilde{\eps} \,\textrm{ for some }\, t<T) \ge 1-p
\end{equation}
\end{theorem}

\paragraph{Convergence to a first-order stationary point} We further compute the time complexity for the LD to converge to a $\eps-$first order stationary point. We define $\x^\star$ to be a $\eps$-first order stationary point if $\|\nabla f(\x^\star)\| \le \eps$.

\begin{theorem}
\label{thm::first_order_convergence}
 Under Assumption \ref{as::grad_lipschitz_ld}, for any $p\in(0,1)$, then with probability at least $1-p$, the time complexity for the LD described in algorithm \ref{alg::LD} to converge to an $\eps$-first order stationary point $\x^\star$ is $\displaystyle \mathcal{O}\left( \frac{\Delta_f d}{ \eps^2 p} \right)$, where $\Delta_f = f(\x_0) - f(\x^\star)$.
\end{theorem}

\paragraph{Convergence to an $\eps$-second-order stationary point}
An $\eps$-second-order stationary point is a more restrictive type of $\eps$-first order stationary point, and is more likely to be an actual local minimizer. 
\begin{definition} 
\label{def::essp}
Consider a smooth function $f(\x)$ with continuous second order derivative. %, where $g(\x)\ll f(\x)$.
A point $\x$ is an $\eps$-second-order stationary point if %to a function $\Phi(\x) = f(\x) + g(\x)$ if
\begin{equation}
    \|\nabla f(\x)\| \le \eps ~\textrm{ and }~ \lambda\big(\nabla^2 f(\x)\big)_{\min} \ge -\eps^2
\end{equation}
where $\lambda(\cdot)_{\min}$ is the smallest eigenvalue.
\end{definition}
We make the strict saddle assumption which is common in nonconvex optimization literature \cite{Ge_EscapeSaddle,lee2016gradient,jin2017escape,constrainedEscapeSaddle18,Lee2019_FirstOrderAvoidSaddle,AvoidSaddle_zeroorderMethod19,HeavyBall_escapesaddle19,liu2018envelope,SSRGD_Li19,Huang_PPD},: i.e.,
\begin{assumption}[strict saddle]
\label{as::strict_saddle_ld}
There exists a constant $q>0 $ such that for all first-order stationary points $\fsp$,  we have
\[
|\lambda(\nabla^2 f(\fsp))| \ge q >0.
\]
\end{assumption}

\begin{assumption}[Hessian Lipschitz]
\label{as::hessian_lipschitz_ld}
$f$ is twice continuously differentiable, and there exists a positive constant $L_2$ such that for all $\x$ and $\y$, $\|\nabla^2 f(\x) - \nabla^2 f(\y)\|\le L_2\|\x-\y\|$.
\end{assumption}

By far in the literature there are two common ways to argue the convergence to second-order stationary points (SSP)
\begin{itemize}
    \item show that $f(\x_T) - f(\x_0) < \Delta_f$ with probabilistic guarantee to ensure the continual function value decrease at saddle point \cite{jin2017escape}
    \item show that $\|\x_T - \x^\star\|$ decreases in the probabilistic sense as $T$ increases \cite{Kleinberg_SGD_escape_local_minima}. 
    
    The time complexity of this approach has the exponential dependency on the inverse of the error tolerance. So in this work we resort to the previous approach.
\end{itemize}

The argument to show sufficient function value decrease from a FSP uses two iterate sequences to demonstrate the continual function value decrease at saddle point. Now that the noise is injected at every iteration, the geometric intuition that the trapping region is thin plus the probabilistic argument should be able to give a similar proof.

In the LD setting we exploit the property of Brownian motion to show the escape from saddle point, i.e. to characterize the perturbed iterate has high probability in the direction of descent, 
\[
(\x_{t} - \x_{\textrm{fsp}})^\trans \nabla^2 f (\x_\textrm{fsp}) (\x_{t} - \x_{\textrm{fsp}}) \le -\zeta 
% \frac{1}{\|\x_{t} - \x_{\textrm{fsp}}\|^2} (\x_{t} - \x_{\textrm{fsp}})^\trans \nabla^2 f (\x_\textrm{fsp}) (\x_{t} - \x_{\textrm{fsp}}) \le -\zeta 
\]

\begin{theorem}
\label{thm::second_order_convergence}
Under Assumptions \ref{as::grad_lipschitz_ld}, \ref{as::strict_saddle_ld} and \ref{as::hessian_lipschitz_ld}, setting the stepsize decay parameter $\nu\in[1,2]$ and $\rho_0=\mathcal{O}(\eps)$, with probability $\mathcal{O}\left( \frac{\eps^{d-1}}{ \Gamma(\frac{d-2}{2}) L^{d-1}q^{d-1} } \right) \cdot \exp(-\mathcal{O}(\eps d))$, the time complexity for the LD described in algorithm \ref{alg::LD} to converge to an $\eps$-second order stationary point $\x^\star$ is $\mathcal{O}\left(\frac{\Delta_f}{\eps^2}\right) + \exp\left(\mathcal{O}(\eps d)\right)$, where $\Delta_f = f(\x_0) - f(\x^\star)$.
\end{theorem}



\begin{table}[H]
\centering
\resizebox{\textwidth}{!}{\begin{tabular}{ lccccc } 
\toprule
method & Bounded & Grad. Lip. & Hess. Lip. & Regularization & others\\
\midrule
\cite{SGLD_Raginsky} & $f$ and $\|\nabla f\|$ & yes & no & $(m,b)$-dissipative &  \shortstack{(1) stoch.\ grad.\ sub-exp.\ tails\ \\ (2) init.\ pt.\  sub-Gauss.\ tails } \\
\cite{SGLD_Gu} & none & yes & no & $(m,b)$-dissipative & none \\
\cite{Hitting_time_analysis_SGLG_ZhangLiangCharikar}& $\|\nabla f\|$ and $\|\nabla^2 f\|$ &  yes &  yes & $(1,0)$-dissipative & grad.\ sub-exp.\ tails  \\
This work & none & yes & yes & Assumption \ref{assumption::regularization_conditions} & strict saddle  \\
\bottomrule
\end{tabular}}
\caption{Comparison between assumptions made for variants of LD optimization schemes. The Hessian Lipschitz assumption is used for second-order convergence property if made.}
% \addtabletext{nomenclature for the TSs refers to the numbered species in the table.}
\label{table::assumptions_summary}
\end{table}
